Performance of a Front End prototype ASIC for picosecond precision time measurements with LGAD sensors

For the High-Luminosity phase of LHC, the ATLAS experiment is proposing the addition of a High Granularity Timing Detector (HGTD) in the forward region to mitigate the effects of the increased pile-up. The chosen detection technology is Low Gain Avalanche Detector (LGAD) silicon sensors that can provide an excellent timing resolution below 50 ps. The front-end read-out ASIC must maintain the performance of the sensor, while keeping low power consumption. This paper presents the results on the first prototype of a front-end ASIC, named ALTIROC0, which contains the analog stages (preamplifier and discriminator) of the read-out chip. The ASIC was characterised both alone and as part of a module with a 2$\times$2 LGAD array of 1.1$\times$1.1 mm$^2$ pads bump-bonded to it. The various contributions of the electronics to the time resolution were investigated in test-bench measurements with a calibration setup. Both when the ASIC is alone or with a bump-bonded sensor, the jitter of the ASIC is better than 20 ps for an injected charge of 10 fC. The time walk effect that arises from the different response of the preamplifier for various injected charges can be corrected up to 10 ps using a Time Over Threshold measurement. The combined performance of the ASIC and the LGAD sensor, which was measured during a beam test campaign in October 2018 with pions of 120 GeV energy at the CERN SPS, is around 40 ps for all measured modules. All tested modules show good efficiency and time resolution uniformity.

==> latex/performance_asic.tex <==
simulation \& test bench with calibration signals 
\begin{itemize}
\item Pulse shape on discri, and TZ/VA probe output, for various amplitude and capacitances 
\item TOA vs Injected charge (probe output amplitude ?) and TOT + correction.
\item Jitter TOA vs injected charge and Cd
\item Jitter probe amplitude vs charge and Cd 
\item probe amplitude vs Cd (fixed injected charge), with 4 channels
\item comparison to simulation ?
\item show probe amplitude for different channels -> see difference due to different path length
\item effect of Cpole? -> minimum effect seen. If flat, not show (Christina)
\end{itemize}


\subsection{Calibration experimental setup}
\label{subsec:setup}

The ALTIROC0 readout board integrates a calibration input for testing the performance of the electronics in a controlled environment. Two identical setups exist at LAL and Omega for calibration measurements. Each setup consists of:
\begin{itemize}
    \item a picosecond generator (ref) 
    \item low voltage power supply for the board
    \item Keithley high voltage power supply for the sensor
    \item splitter for duplication of the generator input signal
    \item Lecroy oscilloscope for waveform sampling
    \item PC for slow control
\end{itemize}

The two setups are shown in Fig.\ref{fig:calibration_setups}. The picosecond generator injects a square pulse of a well defined voltage to the board through a 100fF capacitor, thus producing a very precise injected charge. In parallel, it provides the time reference via the splitter and the acquisition trigger. 

\begin{figure}[htbp]
\centering
\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/setupOmega}}
\hspace*{0.2cm}
\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/setupLAL}}
\caption{ Calibration setup (a) at Omega (b) at LAL}

\label{fig:calibration_setups}
\end{figure}

\subsection{ALTIROC0 readout board}
\label{subsec:board}

The ALTIROC0 readout board has been designed by Omega. It's design has essentially remained the same over the two ASIC versions except from a few minor modifications. The main inputs/outputs that were used for the testing, also illustrated on fig. ,are listed below:

\begin{itemize}
    \item Low voltage power supply input
    \item usb port for slow control transmission
    \item calibration input
    \item Discriminator direct outputs for the 4 channels (choise between VPA and TZ through slow control)
    \item 2 preamplifier probe outputs (choise between preamplifiers/channels through slow control)
\end{itemize}

\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth]{figures/ALTIROCboard_components.png}
\caption{ALTIROC0 readout board and it's main components}
\label{fig:boardComponents}
\end{figure}




\textbf{Jitter measurement: } As shown in Eq. \ref{ec:jitter}, the jitter is expected to be inversely proportional to the injected charge and proportional to the detector capacitance. The relation of the jitter to these parameters was tested experimentaly with the calibration setup. In order to vary the detector capacitance, SMD capacitors were soldered externally to the footprints of the channel inputs. 

The jitter as a function of the injected charge is shown in Fig. \ref{fig:jitterQinj} for a soldered capacitance of 3pF. A 6 ps flat resolution attributed to the generator has been subtracted. The jitter for a charge of 10fC (1 MIP) is found to be 18 ps, while a plateau of 5ps is reached for higher charges. T

The jitter has also been measured for various capacitance values, as shown in Fig. \ref {fig:jitterCs}. As expected, the jitter shows a strong linear dependance to the capacitance, thus justifying the choise of small area sensors with a medium thickness.\\


\begin{figure}[htbp]
\centering



\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/jitter_221118_ALT_V2--Board21_Ch0_VA_ChargeScan_3pF_1K_toaVSprobe}\label{fig:jitterQinj}}
\hspace*{0.2cm}
\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/JitterVsCsoldBoard21_Ch0_VA_Cscan_10fC_1K_discr}\label{fig:jitterCs}}


\caption{(a) jitter as a function of the injected charge for a C$_{sold}$ = 3 pF. \textcolor{red}{also simulation and V1?} (b) Jitter as a function of the soldered capacitance for an injected charge of 10fC. The generator resolution of 6ps has been subtracted quadratically in both measurements.}

\end{figure}


\textbf{Time walk correction:} The accuracy of the time walk correction can also be tested experimentally with calibration. Since the prototype board has two available estimates of the signal amplitude, the time-over-threshold discriminator and the probe amplitude, the time walk correction can be performed using both methods. The time of arrival as a function of the time over threshold and the probe amplitude is shown in Fig. \ref{fig:timewalk} for a soldered capacitance of 3pF. The average residual after correction is found to be in a range of $\pm$ 20 ps using the TOT, while a better performance of $\pm$ 10ps is achieved using the amplitude of the probe.\\


\begin{figure}[htbp]
\centering
%\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/TOAvsTOTcorrected_full}\label{fig:toavstot}}
%\hspace*{0.2cm}
%\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/TOAvsProbeAmpcorrected_full}\label{fig:toavsProbe}}
%\vspace{0.5cm}

\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/toa_vs_tot_221118_ALT_V2--Board21_Ch0_VA_ChargeScan_3pF_1K_probeOff}\label{fig:toavstot}}
\hspace*{0.2cm}
\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/toa_vs_amp_221118_ALT_V2--Board21_Ch0_VA_ChargeScan_3pF_1K_probeOn}\label{fig:toavsProbe}}


\caption{
  Time walk correction for Csold=3pF using (left) the Time-over-threshold discriminator (right) the amplitude of the probe.}

\label{fig:timewalk}

\end{figure}


\textbf{Preamplifier performance comparison:} As described in section \ref{sec:preamp_design}, the prototype integrates two preamplifier types, the transimpedance (TZ) and the voltage (VPA). Both types were tested with calibration. As expected, the VPA signal is higher with a longer fall time. In addition, as shown in  Fig. \ref{fig:vpaVStz_b}, the voltage preamplifier performs slightly better than the transimpedance in terms of jitter. \textcolor{red}{Remove V1 result? Redo for Csold=2,3pF?}   \\

\begin{figure}[htbp]
\centering


\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/ALTV2_avPulse_probeBuf.png}}
\hspace*{0.2cm}
\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/toaRMS_vs_Qinj_V1vsV2_0pF.png}\label{fig:vpaVStz_b}}


\caption{ (a) Average pulse shapes of the VPA and TZ preamplifiers for an injected charge of 10 fC from the preamplifier probe output (b) Jitter as a function of the injected charge for the VPA and TZ preamplifiers of V2 as well as the unoptimized VPA preamplifier of V1.
  }

\label{fig:vpaVStz}

\end{figure}


\textbf{Channel comparison:} The consistency of the electronics' performance has been tested for all the available channels. Figure \ref{fig:allChans} , shows the inverse of the amplitude of the probe as a function of the soldered capacitance. The linear behavior as a function of the capacitance is expected from Eq. \textcolor{red}{add equation}. It has been found, that there is a variation in the performance of the different channels of the order of 15-20\% that is seen both in the probe amplitude and the jitter of the TOA. As shown in Figure \ref{fig:ampVsLength}, this difference is clearly correlated to the length of the connection of the preamplifier input. This can be explained by the fact that the input connection adds to the parasitic capacitance at the input of the preamplifier.


\begin{figure}[htbp]
\centering


\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/Board21_allChans_VA_Cscan_10fC_1K_probe} \label{fig:allChans}}
\hspace*{0.2cm}
\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/InvProbeAmpVsConnectionLengthBoard21_VA_Ampvslength_10fC_1K_0pF}\label{fig:ampVsLength}}


\caption{(a) 1/V$_{out}$ as a function of the soldered capacitance for channels 0-3 of the VPA type (b) 1/V$_{out}$ as a function of the input connection length. Both sets of measurements were performed with an injected charge of 10 fC. }


\end{figure}

\textcolor{red}{Should I add a figure of the jitter for different channels?}

==> latex/performance_lgad.tex <==
\begin{itemize}
\item Bump bonding 
\item Calibration performance (extract the capacitance)
\item TOA vs Injected Q
\item Amplitude probe and jitter probe vs Injected Q
\item Effect of Cpole on signal /performance (probbably to be removed)
\item TOT problem observation
\item Time resolution with probe signal (CFD) 
\item Time resolution with discri using probe amplitude (cut and/or correction) 
\end{itemize}


\subsection{Module assembly}
\textbf{ASIC-sensor interconnection}\\

The interconnection of the sensor to the front-end chip is a critical procedure of the detector assembly process.
Each sensor channel is DC-coupled to the corresponding readout channel on the ASIC through a small (typically \SI{80}{\micro\metre} diameter) solder ball, through an hybridisation process called \textit{bump-bonding}.

The baseline bump-bonding scheme consists of two steps. First under-bump metallization  
(UBM) is performed on both sensor and ASIC pads, as preparation for soldering. Then the solder bump is deposited on the ASIC, and flip-chip is done to position the sensor on top.
%The R\&D effort, presented  below, is being carried out by dedicated groups within the HGTD community.
%For the full HGTD production phase, a combination of private companies and ATLAS institutions is foreseen to share the workload. Suitable companies for the UBM and flip-chip processes have been identified and contacted, and first cost estimates are available. {\TODO Give more general info on who is doing R\&D and production possibility?}

%\textbf{Assembly steps}\\
%Is this a general description or just one possibility as currently done in one of the institutes?
In the hybridisation process, the aluminium pads of the sensor and readout chip are first covered
with NiAu through an auto-catalytic chemical technique.
The bumps are then deposited on the ASICs with a bump deposition machine that places SnAg (or SnPb)
solder balls on the front-end pads and reflows them with an infrared laser system.
The solder bumps are further reflowed in a dedicated machine in order to improve the
placement and the shape uniformity of the bump balls.
Flip-chip, the last step in the hybridisation process, is performed with a S\"uss Microtech bonder
machine with a reflow arm that provides a \SI{0.5}{\micro\metre} placement accuracy and \SI{1}{\micro\metre} post-bond accuracy.
During the bonding cycle the ASICs (with SnAg solder bumps) and the sensors are aligned, heated to \SI{260}{\celsius}
and pressed together lightly.
After flip-chip the assemblies are reflown once again with formic acid.

First studies were performed on a $10 \times 10$ matrix of $1 \times 1$~mm$^2$ pixels in order to prepare for further tests with the ASIC prototype module. 
These preliminary tests confirmed that the critical steps of bump deposition and flip-chip can be conducted successfully with pixel pads \SI{90}{\micro\metre} wide and bump balls of \SI{80}{\micro\metre} diameter. 
In the following step, dummy samples that match mechanically the characteristics of the ASIC prototype modules were assembled obtaining excellent results with a bump strength of 60~g/bump. 
The first HGTD small-scale module prototypes using the first ASIC prototype (\Altirocv{0}\_v1) and LGAD sensors were assembled in summer of 2017. Four assemblies were successfully produced following the baseline procedure used for the previous studies. Two additional modules were assembled using a second iteration of the ASIC, \Altirocv{0}\_v2. {\TODO any difference in the bump-bonding between 2 versions? }

The UBM of the diced chips and only partially diced sensors was done with thicknesses between 4 and \SI{6}{\micro\metre}. 
After bump deposition, the chip solder joints were reflowed and then the flip-chip process with selected sensors
was carried out. 
All bump-bonding cycles were successful, and X-ray inspection indicated good connectivity of all the bump bonds.

An alternative process using Au bumps has also been tested to assemble an LGAD-ASIC module. In this case UBM is not performed, and the gold bumps are deposited one by one on the front-end pads. An additional module was produced and tested using this technique. {\TODO need more info here}


\subsection{Performance with calibration}
\label{subsec:calibSensor}

The calibration setup can accommodate both boards with the ASIC alone or with a flip chip consisting of the sensor bump-bonded to the ASIC. In the latter case, the sensor is not involved in the signal production and only contributes to the electronics input detector capacitance C$_d$.  \\


\textbf{Time-Over-Threshold problem observation:} During the testbeam campaign of June 2018, it was observed that, the time over threshold of the discriminator output is not scaling proportionally with the amplitude of the probe in the case were there is a sensor bump bonded to the asic. Moreover, there is an oscillation on the discriminator falling edge. This problem was verified in testbench with calibration signal, as shown in Fig. \ref{fig:totProblem_b23} . Two possible reasons for this problem have been theorized ; an inductance caused by the length of the pad-sensor HV connection or a coupling of the direct discriminator output to the PCB. In order to investigate the former, a new board with a larger L-shaped HV connection pad has been manufactured. This particular shape of the HV pad allows for many wire bonds to be attached in order to reduce any possible inductance. The degeneration of the falling time for different charges is still present in the modified board for Q$_{inj} <$ 10 fC , however, for higher charges, the problem is reduced, as seen in Fig. \ref{fig:totProblem_b32}.


\begin{figure}[h]
\centering
\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/toeVSprobeAmp_261018_ALT_V2--Board23_Ch0_VA_ChargeScan_1K_probeOn}\label{fig:totProblem_b23}}
\hspace*{0.2cm}
\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/toeVSprobeAmp_211118_Board32_Ch1_VA_ChargeScan_1K_withHV_probeOn}\label{fig:totProblem_b32}}

\caption{ falling time as a function of the probe amplitude for various injected charges for (a) standard HV-connection board (b) L-shaped HV pad board. Both boards are equiped with an asic bump-bonded to an unirradiated 2x2 sensor array. }

\label{fig:totProblem}
\end{figure}



\textbf{Jitter and time walk correction}\\
\begin{figure}[h]
\centering
%\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/TOAvsTOTcorrected_full}\label{fig:toavstot}}
%\hspace*{0.2cm}
%\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/TOAvsProbeAmpcorrected_full}\label{fig:toavsProbe}}
%\vspace{0.5cm}

\subfloat[]{}
\hspace*{0.2cm}
\subfloat[]{\includegraphics[width=0.5\textwidth]{figures/toa_vs_amp_261018_ALT_V2--Board23_Ch0_VA_ChargeScan_1K_probeOn}}


\caption{
  (a) Jitter as a function of the injected charge \textcolor{red}{to be added} (b) residual after the time walk correction. Both measurements were performed on a board with a sensor bump-bonded to the ASIC}

\label{fig:timewalkWithSensor}
\end{figure}


